Blockwise Key Distillation in Satellite-based Quantum Key Distribution

Free-space satellite communication has significantly lower photon loss than terrestrial communication via optical fibers. Satellite-based quantum key distribution (QKD) leverages this advantage and provides a promising direction in achieving long-distance inter-continental QKD. Satellite channels, however, can be highly dynamic due to various environmental factors and time-of-the-day effects, leading to heterogeneous noises over time. In this paper, we compare two key distillation techniques for satellite-based QKD. One is the traditional {\em non-blockwise} strategy that treats all the signals as a whole; the other is a {\em blockwise} strategy that divides the signals into individual blocks that have similar noise characteristics and processes them independently. Through extensive simulation in a wide range of settings, we show trends in optimal parameter choices and when one strategy provides better key generation rates than the other. Our results show that the blockwise strategy can lead to up to $5\%$ key rate improvement (leading to on average $1.9\times10^{7}$ more key bits per day) when considering two types of blocks, i.e., for nighttime and daytime, respectively. The blockwise strategy only requires changes in the classical post-processing stage of QKD and can be easily deployed in existing satellite systems.

==> analysis.tex <==
\section{Sampling-Based Key Analyses} \label{sec:analysis}

%\bing{Just describe the two finite key cases; no need to describe the asymptotic formula.}
%\bing{Introduce effective key rate. Use one paragraph to explain that for a particular setting, we vary the pump power and sampling rate to maximize the effective key rate.}

\subsection{Nonblock-wise Key Analysis}
For the nonblock-wise naive key analysis, the computing the average error over all contact rounds in one day as follows: for any number of block $t$,
\begin{equation}
    Q_{ave} = \frac{1}{B}\bigg(\sum_{i=1}^{t}B_{i}\cdot Q_{i}\bigg),
\end{equation}
% \begin{equation}
%     Q_{ave} = \frac{Q_{n}\cdot N_n + Q_{d}\cdot N_d}{N_{n}+N_{d}},
% \end{equation}
where $Q_{i} = (1-\widetilde{fid}_{ave}^{(i)})/2$ and $\widetilde{fid}_{ave}^{(i)}$ is the average fidelity in each block from Eq. (\ref{eq:fid-ave}). 
% When we have average errors and the number of entanglements over one day, we employ the naive asymptotic secret key analysis to compute a secret key rate as follows:
% %%wb, 12/21/2022, 2h instead of h
% \begin{equation}
%     \Tilde{\keyrate}_{a} = 1 - 2h(Q_{ave}),
% \end{equation}
% where $h(\cdot)$ is the binary entropy. 
For the non-blockwise naive sampling key analysis, we have the following equation to compute a general key rate as follows: for any sampling rate $r\in [0.01,0.5]$, \bing{We may use a much lower sampling rate than 0.01.}
\begin{equation} \label{eq:key-rate-nonblock}
    \Tilde{\keyrate}_{s} = \frac{1}{B}\bigg((B-m)(1-2h(Q_{ave}+\delta))\bigg),
\end{equation}
where $m = r\cdot B$ and $n = B-m$, and $h(x)$ as an extended binary entropy function, namely, $h(x)=-x\log_{2}(x)-(1-x)\log_{2}(1-x)$ if $0\leq x\leq 1/2$, and $h(x)=0$ otherwise. Note that $n(1-2h(Q_{ave}+\delta))$ estimates $n(1-h(Q_{ave}+\delta)) - \lambda_{EC}$ and we may use the $7\%$ sampling rate for this non-blockwise sampling analysis. To compute an effective key rate, we use the following: for any sampling rate $r\in [0.01,0.5]$,
\begin{equation} \label{eq:effective-key-rate-nonblock}
    \Tilde{\keyrate}_{s}^{*} = \frac{1}{N}\bigg((B-m)(1-2h(Q_{ave}+\delta))\bigg),
\end{equation}
where $N$ is the total number of signals that a satellite sends to a pair of ground stations.

\subsection{Block-wise Key Analysis}

Given a block of $N$ raw key bits, an $\epsilon_{sec}$ key may be extracted through a process of error correction and privacy amplification (CITE).  A key is called $\epsilon_{sec}$-secure if it holds that:
\[
\frac{1}{2}\trd{\rho_{SE} - \mathcal{U}_S\otimes\rho_E} \le \epsilon_{sec}.
\]
Above, $\mathcal{U}_S\otimes\rho_E$ represents a uniform random secret key independent of Eve (one may consider this the ``ideal'' system).  A key is $\epsilon_{cor}$ if it holds that the probability Alice's secret key is different from Bob's key is no larger than $\epsilon_{cor}$ (CITE).   Using results from (CITE), it holds that an $\ell$-bit secret key can be generated from the E91 protocol, where:
\begin{equation}
    \ell = n(1 - h(Q + \mu)) - \lambda_{EC} - \log\frac{2}{\epsilon_{sec}^2\epsilon_{cor}},
\end{equation}
where:
\begin{equation}
    \mu = \sqrt{\frac{(n+m)(m+1)}{nm^2}\ln\frac{2}{\epsilon_{sec}}}
\end{equation}
For the block-wise analysis, we consider can break the $N$ raw key signal into $B$ blocks of size $B_i$.  Each block is sampled from independently using $m_i$ samples.  Then, it can be shown that the total secret key size will be:
\begin{equation}
    \ell = \sum_i(B_i-m_i)(1 - h(q_i + \mu_i)) - \lambda_{EC},
\end{equation}
where $\mu_i$ is the above $\mu$ function, but using $n = B_i - m_i$ and $m = m_i$.  We assume, later, in our evaluations that $\lambda_{EC} = \sum_i(B_i-m_i)h(q_i + \mu_i)$.
%
Therefore, the effective key rate is 
\begin{equation}\label{eq:effective-keyrate-time-approx}
    \keyrate_s^{*} = \frac{1}{N}\left(\sum_{i=1}^t(B_i - m_i)(1 - 2h(q_i + \delta_i)) \right),
\end{equation}
where $N$ is the total number of signals that a satellite sends to a pair of ground stations.


% In this case, the asymptotic key rate for the nighttime and daytime, computing the average key rate is as follows:
% \begin{equation}\label{eq:simple-block-key-rate}
%     \keyrate_{a} = \frac{1}{B}\bigg(\sum_{i=1}^{t}B_{i}(1-2h(Q_{i}))\bigg),
% \end{equation}
% where $t$ is the number of blocks. 


%%wb, 3/31/2023, use the new formula above
\iffalse 
\begin{theorem}
For instance, one can use methods from \cite{yao2020quantum} to derive new secure key-rate bounds in this scenario resulting in a secret key rate of: for any number of blocks $t$,
\begin{equation}\label{eq:keyrate-time1}
    \keyrate_s = \frac{1}{B}\left(\sum_{i=1}^t(B_i - m_i)(1 - h(q_i + \delta_i)) - \lambda_{EC}\right),
\end{equation}
where $t$ is the number of blocks and the sampling error $\delta_{i}$ is as follows: for each key pool $B_{i}$,
\begin{equation*}
    \delta_{i} = \sqrt{\frac{(m_{i}+n_{i}+2)\ln{(2/\varepsilon^{2})}}{m_{i}(m_{i}+n_{i})}},
\end{equation*}
where an epsilon $\varepsilon$ is $10^{-36}$ and $m_{i}$ is the sampling size on generated entanglements in each pool, $B_{i} = m_{i}+n_{i}$, namely $B_{i}$ is $N_{t}$.
\end{theorem}
\begin{proof}
Hello.
\end{proof}
\fi 

\bing{4/5/2023: based on the above, $m_i$ needs to be sufficiently large. $\delta$ is 0.04, 0.013, 0.004 when $m$ is $10^5$, $10^6$, and $10^7$, respectively.}

==> blockwise-res.tex <==
\subsection{Blockwise Finite Key Results}
We next present the results when using the blockwise key distillation scheme. 

Plots (6 curves for night and day separately): 
(i) x-axis: distance (600, 1200, 1800), y-axis: optimal pump power. 6 curves: for the day/night and altitude combination. Please use coloring scheme: 
\begin{itemize}
    \item Use blue for altitude of 500 km, cross dashed lines for nighttime and circle solid lines for daytime.
    \item Use red for altitude of 800 km, cross dashed lines for nightime and circle solid lines for daytime.
    \item Use black for altitude of 1000 km, cross dashed lines for nightime and circle solid lines for daytime.
\end{itemize}

(ii) x-axis: distance (600, 1200, 1800), y-axis: success probability.  6 curves.

(iii) x-axis: distance (600, 1200, 1800), y-axis: fidelity.  6 curves.

(iv) x-axis: distance (600, 1200, 1800), y-axis: total number of entanglements for night and day separately. 6 curves.

(v) x-axis: distance (600, 1200, 1800), y-axis: number of secret keys for night and day separately. 6 curves.

\begin{figure*}[ht]
    \centering
    \subfigure[optimal pump power]{\includegraphics[width=0.20\textwidth]{images/bk_sampling_pump_powers_overhead_1_1.png}}
    \hspace{-.5cm}
    \subfigure[success pr.]{\includegraphics[width=0.20\textwidth]{images/bk_sampling_psucc_overhead_1_1.png}} 
    \hspace{-.5cm}
    \subfigure[fidelity]{\includegraphics[width=0.20\textwidth]{images/bk_sampling_fid_ave_overhead_1_1.png}}
    \hspace{-.5cm}
    \subfigure[\# of ent.]{\includegraphics[width=0.20\textwidth]{images/bk_sampling_num_ents_overhead_1_1.png}}
    \hspace{-.5cm}
    \subfigure[\# of keys]{\includegraphics[width=0.20\textwidth]{images/bk_sampling_num_keys_overhead_1_1.png}}
    \caption{Results for the blockwise distillation scheme (1 day).  }
    % \label{fig:foobar}
\end{figure*}

%%wb, 3/31/2023, comment out bisect mode
\iffalse 
\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=0.24\textwidth]{images/bk_sampling_pump_powers_bisect_1_1.png}} 
    \subfigure[]{\includegraphics[width=0.24\textwidth]{images/bk_sampling_psucc_bisect_1_1.png}} 
    \subfigure[]{\includegraphics[width=0.24\textwidth]{images/bk_sampling_fid_ave_bisect_1_1.png}}
    \subfigure[]{\includegraphics[width=0.24\textwidth]{images/bk_sampling_num_ents_bisect_1_1.png}}
    \caption{Blockwise sampling simulation results—bisect mode (a) Optimal pump power (b) Successful probability (c) Average fidelity (d) The number of entanglements.}
    % \label{fig:foobar}
\end{figure}
\fi 

\iffalse 
\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_sampling_total_num_ents_overhead_1_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_sampling_noise_ave_overhead_1_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_sampling_total_num_keys_overhead_1_1.png}}
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_sampling_total_num_ents_bisect_1_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_sampling_noise_ave_bisect_1_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_sampling_total_num_keys_bisect_1_1.png}}
    \caption{Blockwise sampling key distillation results (a) Overhead—The total number of entanglements (b) Overhead—Average noise (c) Overhead—The number of keys, (a) Bisect—The total number of entanglements (b) Bisect—Average noise (c) Bisect—The number of keys..}
    \label{fig:bk-sampling-key-distillation}
\end{figure}
\fi


==> model-simulator.tex <==
\section{Model and Simulator}\label{sec:model}

In this work we consider a grid network consisting of $N\times N$ nodes with each node connected to at most four others, their immediate neighbors up, down, left, and right.  These connections represent fiber links allowing for the direct transmission of qubits between neighboring nodes only.  We assume a classical communication network allowing any pair of nodes to send classical messages.  We do not assume this communication is secret; however for all user and trusted node communication we do assume it is authenticated.  Each node in this network may be either a User (Alice or Bob); a Trusted Node; or a Quantum Repeater.  We place Alice at the lower-left corner of the network and Bob in the upper-right (thus, these users have only two neighbors they are connected to).  Later, we will simulate alternative numbers and locations of the trusted nodes; however, predominately the other nodes will consist of quantum repeaters in contrast to current day QKD networks.

\triplefig{stage1.pdf}{Initial network}{stage2.pdf}{Stage 1}{stage3.pdf}{Stage 2}{(a) The initial network of a $5\times5$ grid, with a central trusted node ($T$) between Alice ($A$) and Bob ($B$). (b) A possible network configuration after stage 1, in which some nodes succeed in establishing a shared state of the form in Equation (\ref{eq:shared-state0}) with their neighbors over the fiber channels and some do not. 
%Note that there are a number of possible paths between A, B and T. 
(c) Successful entanglement chaining and routing (depicted as the ``internal links'' at repeaters) as discussed in Stage 2. In this graph, routing has resulted in end-to-end paths being created between each pair of $A$, $B$ and $T$. These routes are successful only if every Bell state measurement along the path succeeds. Furthermore, the probability of decoherence increases with the path length in our model as discussed; thus minimizing the path lengths through effective routing algorithms and trusted nodes is advantageous.  See also Figure \ref{fig:guide}.}{stages1-3}

%%intra-repeater connections

\begin{figure}
    \centering
    \includegraphics{sideguide.pdf}
    \caption{A legend for our network diagrams. Left: (a) denotes a node in the network, specifically a repeater with 4 (b) connection terminals from which entangled photons are sent and received over (c) fiber optic connections between other repeaters and (d) trusted nodes. Right: an entangled channel (e) connecting multiple trusted nodes through intra-node entanglement (f).}
    \label{fig:guide}
\end{figure}

Users and trusted nodes perform the E91 QKD protocol.  For notation, we assume there are $n$ trusted nodes denoted $T_1, \ldots, T_n$.  We label Alice as $T_0$ and Bob as $T_{n+1}$.  For every pair of users and trusted nodes there exists a private raw-key pool; that is, for every $i,j \in \{0,\cdots, n+1\}$, with $i < j$, there exists a buffer $\rawkey_{i,j}$, storing the raw key shared between nodes $T_i$ and $T_j$.  Note that repeaters do not have key buffers.  As we are using the entanglement based E91 protocol, the first goal of the network is to establish joint entanglement between these pairs of nodes $T_i$ and $T_j$, ideally the Bell state $\ket{\Phi^+} = \frac{1}{\sqrt{2}}(\ket{00} + \ket{11})$.  This resource may be used to establish a secret key between users.

The quantum network we analyze operates in {\em rounds}, each round consisting of {\em three primary stages} (see examples in Figures \ref{fig:stages1-3} and \ref{fig:guide}).  The first stage, and part of the second stage, are standard in repeater-only quantum networks (see \cite{pant2019routing,chakraborty2019distributed}). As mentioned, nodes have at most four inputs into them (since the two users are at the corner of grid, they each only have two inputs); we assume that nodes have the capability of storing a single qubit in short-term memory for each of these inputs, through one complete round.  After the round is complete, any qubits not measured, are discarded.  That is, the memory capabilities of nodes are not sufficient to store a qubit through two or more rounds in our network.  Note that users in our network have the fewest demands on quantum memory.

In the first stage, adjacent nodes attempt to share an entangled pair, in particular the Bell state $\ket{\Phi^+}$, with one particle remaining at a local node and the other being transmitted to an adjacent node.  Due to fiber loss, this succeeds with a certain probability $p = 10^{-\alpha L/10}$ where $\alpha$ is the fiber attenuation coefficient (we use $\alpha = .15$ in our later simulations).  Furthermore, even if successful, the entangled pair may not be a Bell state $\ket{\Phi^+}$ but instead will, with probability $D$, depolarize and become completely mixed.  Ultimately, after this first stage, adjacent nodes $u$ and $v$ will either not have any qubit in their short-term memory (with probability $1-p$) or, with probability $p$, they will share a quantum state of the form:
\begin{equation}\label{eq:shared-state0}
\rho_{u,v} = (1-D)\kb{\Phi^+} + D \cdot \frac{I}{4},
\end{equation}
where $I$ is the identity operator on two qubits.  Note this $D$ may be used to model channel noise along with noise internal to the quantum memory of the repeater.  As is standard in repeater-network analyses \cite{pant2019routing,chakraborty2019distributed}, we assume that nodes are able to determine whether a qubit has arrived in their short-term quantum memory or if it is a vacuum.

In the second stage, a routing protocol, to be discussed (see Section~\ref{sec:routing}), is performed to decide how to %optimally 
effectively route entanglement between nodes $T_i$ and $T_j$ for $i \ne j$.  This routing protocol can take into account whether nodes have a qubit in their short-term memory.  The goal of this stage, and in particular the routing algorithm, is to determine a set of paths, the end-points of which are either users or trusted nodes, while the interior nodes of each path are quantum repeaters.  Given these paths, the quantum repeaters will perform entanglement swapping operations on the qubits that are locally held in their short-term memory, which, if successful, create ``virtual'' entangled links between the end-points of each path.
%attempting to create an end-to-end entangled pair between the end-points of each path.  
The entanglement swapping operations at the repeaters, which themselves consist of Bell measurements, succeed only with a certain probability that we denote as $B$.  We assume the network is able to determine whether a successful entanglement swapping occurred or not.  Thus, at the end of this stage, end-nodes $T_i$ and $T_j$ on each path can determine whether the network was successful in creating an end-to-end  path between these nodes.  Note that they cannot tell if the state they share is the correct Bell state $\ket{\Phi^+}$ or the completely mixed state $I/4$ due to depolarization.  At this point, repeaters are no longer needed until the next round, and users and trusted nodes share a state of the form in Equation (\ref{eq:shared-state}), where the probabilities of the mixed state depend on $D$ and the path length -- in particular, on a path consisting of $k$ interior nodes, the shared state will either be:
\begin{equation}\label{eq:shared-state}
\rho_{T_iT_j} = (1-D)^{k+1}\kb{\phi^+} + (1-[1-D]^{k+1})\cdot\frac{I}{4},
\end{equation}
or a vacuum if one or more repeaters failed in their entanglement swapping operation.

Finally, in the third stage, all pairs $T_i$ and $T_j$ of users and trusted nodes which have a shared state, and not a vacuum, attempt to distill a raw-key bit using the E91 QKD protocol.  If successful (which depends on users choosing the correct basis, and as such it is successful with probability $1/2$), the key-bit is added to a local raw key-pool for those users $\rawkey_{i,j}$.  Any qubit that was not measured by now is discarded and the network repeats at stage 1, attempting to establish fresh entangled pairs between adjacent nodes.  Refer to Figures \ref{fig:stages1-3} and \ref{fig:guide}.

We wrote a custom simulator to simulate the behavior of this network and these three stages.  This simulator maintains a raw-key pool $\rawkey_{i,j}$ between each pair of users $T_i$ and $T_j$ as would be done in an actual operation of this network.  In practice, nodes $T_i$ and $T_j$ will, once the length of the raw key in $\rawkey_{i,j}$ is sufficiently large, perform error correction and privacy amplification, leading to a secret key of size $|\secretkey_{i,j}|$.  In our simulations, we are interested in the theoretical performance of this network, and so we only do this process once at the end of the simulation and set $|\secretkey_{i,j}| = |\rawkey_{i,j}|\cdot (1-2h(Q))$ where $Q$ is the error in the raw key pool $\rawkey_{i,j}$ and where $h(x)=x\log(x)-(1-x)\log(1-x)$ is the binary entropy function. Again, as we are only interested in theoretical behavior, we compute $Q$ based on the actual simulator data; in practice $Q$ may be estimated by sampling from $\rawkey_{i,j}$.

Of course, the ultimate goal of the network is to maximize the secret key pool between Alice and Bob (i.e., $T_0$ and $T_{n+1}$).  If $n=0$ (i.e., there is no trusted node), at this point, we are done.  However for $n\ge 1$, a final key-routing process is required of the trusted nodes who must attempt to ``push'' a maximal amount of key material to Alice and Bob.  For $n=1$, this is trivial: $T_1$ will simply broadcast $\secretkey_{0,1}\oplus \secretkey_{1,2}$ (here, $T_0$ is Alice and $T_2$ is Bob); if they are not of equal length, then only the left-portion is broadcast.  Alice and Bob already have a secret key of size $|\secretkey_{0,2}|$ before this process.  Thus, finally, they end up with a secret key of total size $|\secretkey_{0,2}| + \min(|\secretkey_{0,1}|, |\secretkey_{1,2}|)$.  When $n > 1$ the situation is more complicated; in this work we use the max-flow algorithm to determine how many additional bits are appended to $\secretkey_{0,n+1}$.  Note that, at the end, not all key bits in trusted node pools may be usable if there is an insufficient amount of key material in ``matching'' nodes.  Later, when we evaluate performance of our routing protocols, we will look at the key-rate of the network, namely the size of the final secret key between Alice and Bob (after the trusted nodes perform this final key-routing process) divided by the total number of network rounds.  



==> nonblock-asymp-res.tex <==
\subsection{Nonblock Asymptotic Results}
Basic statistics:
For the 3 $\times$ 3 altitude and baseline combinations, list 
\begin{itemize}
    \item the orbit time (amount of time to finish one orbit; this only depends on the altitude, does not depend on baseline); 
    \item the number of passes in night time and the number of passes in day time;
    \item for each pass at night, the duration of the pass time (i.e., the contact length, i.e., the duration that the satellite is in the contact of both ground stations). Similarly, do this for day time. 
\end{itemize} 

As a baseline distance increases between two ground stations, the contact length, a passing time between a satellite and the ground stations, decreases for every altitude and orbital mode (see Tables \ref{table:1}, \ref{table:2}, and \ref{table:3}). Particularly, the passing time of the altitude of 500 km and the distance of 1922 km in overhead mode significantly drops, which is 23 seconds (see table \ref{table:1}).




Plots (6 curves for night and day separately): 
(i) x-axis: distance (551, 1200, 1922), y-axis: optimal pump power. 6 curves: for the day/night and altitude combination. Please use coloring scheme: 
\begin{itemize}
    \item Use blue for altitude of 500 km, cross dashed lines for nighttime and circle solid lines for daytime.
    \item Use red for altitude of 800 km, cross dashed lines for nightime and circle solid lines for daytime.
    \item Use black for altitude of 1000 km, cross dashed lines for nightime and circle solid lines for daytime.
\end{itemize}

(ii) x-axis: distance (551, 1200, 1922), y-axis: success probability.  6 curves.

(iii) x-axis: distance (551, 1200, 1922), y-axis: fidelity.  6 curves.

(iv) x-axis: distance (551, 1200, 1922), y-axis: total number of entanglements for night and day separately. 6 curves.

% \begin{figure}[H]
%     \centering  \includegraphics[width=0.5\textwidth]{images/nbk_asymp_data_00.png}
%     \caption{Non-blockwise asymptotic data of nighttime and daytimes—optimal pump powers, successful probabilities, average fidelities, and numbers of entanglements.}
%     \label{fig:nbk_asymp_data_00}
% \end{figure}

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=0.24\textwidth]{images/nbk_asymp_pump_powers_overhead_1.png}} 
    \subfigure[]{\includegraphics[width=0.24\textwidth]{images/nbk_asymp_psucc_overhead_1.png}} 
    \subfigure[]{\includegraphics[width=0.24\textwidth]{images/nbk_asymp_fid_ave_overhead_1.png}}
    \subfigure[]{\includegraphics[width=0.24\textwidth]{images/nbk_asymp_num_ents_overhead_1.png}}
    
    \caption{Non-blockwise asymptotic simulation results—overhead mode (a) Optimal pump power (b) Successful probability (c) Average fidelity (d) The number of entanglements. \bing{3/20/2023: When optimizing pump power, I think we should also allow the choice of 0. This will not affect the total number of keys for the blockwise approach, but will be helpful to the non-blockwise approach. }}
    \label{fig:nbk_asymp_data_00}
\end{figure}

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=0.24\textwidth]{images/nbk_asymp_pump_powers_bisect_1.png}} 
    \subfigure[]{\includegraphics[width=0.24\textwidth]{images/nbk_asymp_psucc_bisect_1.png}} 
    \subfigure[]{\includegraphics[width=0.24\textwidth]{images/nbk_asymp_fid_ave_bisect_1.png}}
    \subfigure[]{\includegraphics[width=0.24\textwidth]{images/nbk_asymp_num_ents_bisect_1.png}}
    \caption{Non-blockwise asymptotic simulation results—bisect mode (a) Optimal pump power (b) Successful probability (c) Average fidelity (d) The number of entanglements.}
    \label{fig:nbk_asymp_data_01}
\end{figure}

For every altitude and orbital mode, the number of entangled states declines as the distance between the two ground stations grows because the passing time and the successful probability decline. Specifically, in the overhead mode with an altitude of 500 km and a distance of 1922 km, the number of entanglements sinks because its passing time is significantly dropped, see Fig \ref{fig:nbk_asymp_data_00} and Table \ref{table:1}.\\

Plots (3 curves for night and day together): 
(i) x-axis: distance (551, 1200, 1922), y-axis: total number of entanglements for a day. This only has 3 curves. Use blue for altitude of 500 km, use red for altitude of 800 km, use black for altitude of 1000 km. Use solid lines with different marks for the three cases.

(ii) x-axis: distance (551, 1200, 1922), y-axis: average error rate (in a day). This only has 3 curves.

(iii) x-axis: distance (551, 1200, 1922), y-axis: total number of secret keys  (in a day). This only has 3 curves.

% \begin{figure}[H]
%     \centering  \includegraphics[width=0.5\textwidth]{images/nbk_asymp_data_01.png}
%     \caption{Non-blockwise asymptotic data—the total number of entanglements, the average noise, and the number of secret keys.}
%     \label{fig:nbk_asymp_data_01}
% \end{figure}

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/nbk_asymp_total_num_ents_overhead_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/nbk_asymp_noise_ave_overhead_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/nbk_asymp_total_num_keys_overhead_1.png}}
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/nbk_asymp_total_num_ents_bisect_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/nbk_asymp_ave_error_bisect_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/nbk_asymp_num_keys_bisect_1.png}}
    \caption{Non-blockwise asymptotic key distillation results (a) Overhead—The total number of entanglements (b) Overhead—Average noise (c) Overhead—The number of keys, (d) Bisect—The total number of entanglements (e) Bisect—Average noise (f) Bisect—The number of keys.}
    % \label{fig:foobar}
\end{figure}

% \begin{figure}
%     \centering
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/nbk_asymp_total_num_ents_bisect_1.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/nbk_asymp_ave_error_bisect_1.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/nbk_asymp_num_keys_bisect_1.png}}
%     \caption{Non-blockwise asymptotic key distillation results—bisect mode (a) The total number of entanglements (b) Average noise (d) The number of keys. }
%     % \label{fig:foobar}
% \end{figure}

As the distance between the two ground stations grows, the number of secret keys plunges  because the number of entanglements and the average noise fail for every altitude and orbital mode. Especially in the overhead mode with an altitude of 500 km and a distance of 1922 km, the number of keys slopes drastically  because the number of entanglements is significantly tumbled, see Fig \ref{fig:nbk_asymp_data_01}.\\
  


==> nonblockwise-res.tex <==
\subsection{Nonblockwise Finite Key Results}
We next present the results when using the nonblockwise key distillation scheme. 

\begin{figure*}[ht]
    \centering
    \subfigure[optimal pump power]{\includegraphics[width=0.20\textwidth]{images/nbk_sampling_pump_powers_overhead_1_1.png}}
    \hspace{-.5cm}
    \subfigure[success pr.]{\includegraphics[width=0.20\textwidth]{images/nbk_sampling_psucc_overhead_1_1.png}} 
    \hspace{-.5cm}
    \subfigure[fidelity]{\includegraphics[width=0.20\textwidth]{images/nbk_sampling_fid_ave_overhead_1_1.png}}
    \hspace{-.5cm}
    \subfigure[\# of ent.]{\includegraphics[width=0.20\textwidth]{images/nbk_sampling_num_ents_overhead_1_1.png}}
    \hspace{-.5cm}
    \subfigure[\# of keys]{\includegraphics[width=0.20\textwidth]{images/nbk_sampling_total_num_keys_overhead_1_1.png}}
    \caption{Results for the non-blockwise distillation scheme (1 day). }
    % \label{fig:foobar}
\end{figure*}

==> optimization.tex <==
\section{Optimizations}
 \bing{This section can be removed.}
\subsection{Finding an Optimal Laser Pump Power:Nonblock Mode}
We find the set of optimal laser pump powers, $\boldsymbol{n^{*}_{s}}$ in the nonblock-asymptotic mode, for all time blocks and sets of laser pump powers $\boldsymbol{n_{s}} = n_{s}^{(1)},...,n_{s}^{(t)}$,
\begin{equation}
    \argmax_{\boldsymbol{n_{s}}} \mathcal{F} \defeq \Big\{\boldsymbol{n_{s}} \in \mathcal{N}: \mathcal{F}(\boldsymbol{n_{s}}) = \sup_{\mathcal{N}}\mathcal{F}\Big\},
\end{equation}
where $\mathcal{N}$ is a range of possible laser pump powers, i.e., $\mathcal{N}=[0.001,0.1]$ and $\mathcal{F}$ is a function computing the number of secure keys, namely:
\begin{equation}
    \mathcal{F}\big(\boldsymbol{n_{s}}\big) \defeq B\cdot (1-2h(Q_{ave})),
\end{equation}
where $B=B(\boldsymbol{n_{s}}) = \sum_{i=1}^{t}B_{i}$, $B_{i} = S_{\#}\cdot Psucc(n_{s}^{(i)})$, and $Q_{ave} = \sum_{i=1}^{t}B_{i}\cdot Q_{ave}(n_{s}^{(i)})/B$, $Q_{ave}(n_{s}^{(i)}) = \big(1-fid_{ave}(n_{s}^{(i)})\big)/2$.

We find the set of optimal laser pump powers, $\boldsymbol{n^{*}_{s}}$ in the nonblock-sampling finite mode, for all time blocks and sets of laser pump powers $\boldsymbol{n_{s}} = n_{s}^{(1)},...,n_{s}^{(t)}$,
\begin{equation}
    \argmax_{\boldsymbol{n_{s}}} \mathcal{F} \defeq \Big\{\boldsymbol{n_{s}} \in \mathcal{N}: \mathcal{F}(\boldsymbol{n_{s}}) = \sup_{\mathcal{N}}\mathcal{F}\Big\},
\end{equation}
where $\mathcal{N}$ is a range of possible laser pump powers, i.e., $\mathcal{N}=[0.001,0.1]$ and $\mathcal{F}$ is a function computing the number of secure keys, namely:
\begin{equation}
    \mathcal{F}\big(\boldsymbol{n_{s}}\big) \defeq n\cdot (1-2h(Q_{ave}+\delta)),
\end{equation}
where $n=B-m$, $ B=B(\boldsymbol{n_{s}})=\sum_{i=1}^{t}B_{i}$, $B_{i} = S_{\#}\cdot Psucc(n_{s}^{(i)})$, $m$ is the size of samples in $B$, $\delta$ is a sampling error in $m$, and $Q_{ave} = \sum_{i=1}^{t}m_{i}\cdot Q_{ave}(n_{s}^{(i)})/m$, $Q_{ave}(n_{s}^{(i)}) = \big(1-fid_{ave}(n_{s}^{(i)})\big)/2$.
\subsection{Finding an Optimal Laser Pump Power: Block Mode}
We find an optimal laser pump power, $n_{s}^{*}$, for a satellite laser photon generator as follows: for each time period, e.g., nighttime, daytime and for any a pump power $n_{s}\in \mathcal{N}$,
\begin{equation}
    \argmax_{n_s} \mathcal{F} \defeq \Big\{n_s \in \mathcal{N}: \mathcal{F}(n_s) = \sup_{\mathcal{N}}\mathcal{F}\Big\},
\end{equation}
where $n_{s}$ is a laser pump power, $\mathcal{N}$ is a range of possible laser pump powers, i.e., $\mathcal{N}=[0.0001,0.1]$, and $\mathcal{F}$ is a function computing the number of secure keys, namely:
\begin{equation}
    \mathcal{F}(n_{s})\defeq B(n_{s})\cdot\Big(1-2h\big(Q_{ave}(n_{s})\big)\Big),
\end{equation}
where $B(n_{s}) = R_{\#}\cdot(S_{\#}\cdot Psucc_{tot}(n_{s}))$ and $Q_{ave}(n_{s}) = (1-fid_{ave}(n_{s}))/2$. Note that $R_{\#}$ is the number of satellite contact rounds during the time period, and $S_{\#}$ is the number of signals per second, e.g., $10^{9}/sec$, to make entanglement quantum states. For example, a set of grounds stations can receive the number of $S_{\#}\cdot Psucc_{tot}(n_{s})$ of entanglements by one passing time of satellite contact and have the number of $R_{\#}\cdot(S_{\#}\cdot Psucc_{tot}(n_{s}))$ of entanglements during the time period. When we use the finite-sampling key analysis, the function is replaced by:
\begin{equation}
    \mathcal{F}(n_{s})\defeq \Big(B(n_{s})-m\Big)\cdot\Big(1-2h\big(Q_{ave}(n_{s})+\delta\big)\Big),
\end{equation}
where $m$ is the sampling size out of the number of entanglements $B(n_{s})$ and $\delta$ is a sampling error. Once we find an optimal pump power $n_{s}^{*}$, then we can set it as the optimal pump power $Ns$ for the time period. 
% \subsection{Finding an Optimal Pump Power: Block-wise Model}

\subsection{Finding an Optimal Sampling Rate}

==> perf-old.tex <==
\section{Performance Evaluation} \label{sec:perf}
%We are now in a position to evaluate the performance of the proposed QKD network using our various routing algorithms. We will compare the performance of each algorithm in number of different scenarios and configurations, and attempt to draw lessons about

To estimate $\lambda_{EC}$ in Eq.(\ref{eq:keyrate-time1}), we use the following equation for simulations to compute a general key rate, namely:
\begin{equation}\label{eq:keyrate-time-approx}
    \keyrate_s = \frac{1}{B}\left(\sum_{i=1}^t(B_i - m_i)(1 - 2h(q_i + \delta_i)) \right),
\end{equation}
where $B$ is the total number of entanglements that ground stations received.
To compute a effective key rate, we use the following:
\begin{equation}\label{eq:effective-keyrate-time-approx}
    \keyrate_s^{*} = \frac{1}{N}\left(\sum_{i=1}^t(B_i - m_i)(1 - 2h(q_i + \delta_i)) \right),
\end{equation}
where $N$ is the total number of signals that a satellite sends to ground stations. \bing{Should this be in the previous section?} \\
In this section, we evaluate the performance xx. 

bisect and overhead modes.

ground station distance: 551 km—Tronto and NYC, 1200 km—Lijiang and Delingha, and 1922 km—Houston and Washington, D.C.

Satellite altitude: 500 km, 800 km, 1000 km

nighttime $P_d$: $3 \times 10^{-6}$

day time $P_d$: $3 \times 10^{-3}$

Ignore $p_2$ in simulation; not ignore $p_2$ in simulation. We define the nighttime as 10 hours, and so the daytime as 14 hours.


\begin{table}[h!]
\centering
% \begin{tabular}{ |p{2.5cm}||p{1.5cm}|p{1.5cm}|p{1.5cm}|  }
\begin{tabular}{ |c||c|c|c|  }
 \hline
 \multicolumn{4}{|c|}{altitude = 500 km \& overhead mode} \\
 \hline
orbit time = 5647 sec & b=551 km & b=1200 km & b=1922 km\\
 \hline
  the contact length & 217 sec & 125 sec&  23 sec\\
 \hline
num of passes-night  & 7  &7&   7\\
\hline
num of passes-day  & 9    &9&   9\\
 \hline
 \multicolumn{4}{|c|}{altitude = 500 km \& bisect mode} \\
 \hline
orbit time = 5647 sec & b=551 km & b=1200 km & b=1922 km\\
 \hline
  the contact length & 284 sec & 241 sec&  115 sec\\
 \hline
num of passes-night  & 7  &7&   7\\
\hline
num of passes-day  & 9    &9&   9\\
 \hline
\end{tabular}
\\
\caption{The basic statistics of the 1-day satellite round with an altitude of 500 km.}
\label{table:1}
\end{table}

\begin{table}[h!]
\centering
% \begin{tabular}{ |p{2.5cm}||p{1.5cm}|p{1.5cm}|p{1.5cm}|  }
\begin{tabular}{ |c||c|c|c|  }
 \hline
 \multicolumn{4}{|c|}{altitude = 800 km \& overhead mode} \\
 \hline
orbit time = 6022 sec & b=551 km & b=1200 km & b=1922 km\\
 \hline
  the contact length & 365 sec & 268 sec&  159 sec\\
 \hline
num of passes-night  & 6  & 6 &   6\\
\hline
num of passes-day  & 9    & 9 &   9\\
 \hline
 \multicolumn{4}{|c|}{altitude = 800 km \& bisect mode}\\
 \hline
orbit time = 6022 sec & b=551 km & b=1200 km & b=1922 km\\
 \hline
  the contact length & 441 sec & 411 sec&  344 sec\\
 \hline
num of passes-night  & 6  & 6 &   6\\
\hline
num of passes-day  & 9    & 9 &   9\\
 \hline
\end{tabular}
\\
\caption{The basic statistics of the 1-day satellite round with an altitude of 800 km.}
\label{table:2}
\end{table}

%%wb, 3/10/2023, results for Nonblock asymptotic results
\input{nonblock-asymp-res}

\input{blockwise-res}

\subsection{Selecting Optimal Pump Power}

\subsubsection{Satellite Altitude 500 km}
Plot how the number of entanglement, fidelity and the total number of keys (plot blockwise and non-blockwise separately, show the result under optimal sampling) as a function of pump power; main message: pump power has roughly opposite impact on the number of entanglement and fidelity; finding optimal pump power is important. 


4*2*2 (bisect and overhead mode; night time daytime) figures in total; in each figure, plot 3 curves (3 distance values).

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_ents_overhead_500_night_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_fid_aves_overhead_500_night_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_key_overhead_500_night_1.png}}
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_ents_overhead_500_day_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_fid_aves_overhead_500_day_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_key_overhead_500_day_1.png}}
    \caption{Optimal pump power results with 500 km altitude—overhead mode: (a) the number of entanglement—nighttime, (b) the average fidelity—nighttime, (c) the number of keys—nighttime, (d) the number of entanglement—daytime, (e) the average fidelity—daytime, (f) the number of keys—daytime}
     \label{fig:op_pump_power_overhead_500}
\end{figure}

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_ents_bisect_500_night_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_fid_aves_bisect_500_night_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_key_bisect_500_night_1.png}}
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_ents_bisect_500_day_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_fid_aves_bisect_500_day_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_key_bisect_500_day_1.png}}
    \caption{Optimal pump power results with 500 km altitude—bisect mode: (a) the number of entanglement—nighttime, (b) the average fidelity—nighttime, (c) the number of keys—nighttime, (d) the number of entanglement—daytime, (e) the average fidelity—daytime, (f) the number of keys—daytime}
     \label{fig:op_pump_power_bisect_500}
\end{figure}


% \newpage


\subsubsection{Satellite Altitude 800 km}

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_ents_overhead_800_night_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_fid_aves_overhead_800_night_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_key_overhead_800_night_1.png}}
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_ents_overhead_800_day_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_fid_aves_overhead_800_day_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_key_overhead_800_day_1.png}}
    \caption{Optimal pump power results with 800 km altitude—overhead mode: (a) the number of entanglement—nighttime, (b) the average fidelity—nighttime, (c) the number of keys—nighttime, (d) the number of entanglement—daytime, (e) the average fidelity—daytime, (f) the number of keys—daytime}
     \label{fig:op_pump_power_overhead_800}
\end{figure}

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_ents_bisect_800_night_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_fid_aves_bisect_800_night_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_key_bisect_800_night_1.png}}
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_ents_bisect_800_day_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_fid_aves_bisect_800_day_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_key_bisect_800_day_1.png}}
    \caption{Optimal pump power results with 800 km altitude—bisect mode: (a) the number of entanglement—nighttime, (b) the average fidelity—nighttime, (c) the number of keys—nighttime, (d) the number of entanglement—daytime, (e) the average fidelity—daytime, (f) the number of keys—daytime}
     \label{fig:op_pump_power_bisect_800}
\end{figure}

% \newpage

\subsubsection{Satellite Altitude 1000 km}

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_ents_overhead_1000_night_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_fid_aves_overhead_1000_night_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_key_overhead_1000_night_1.png}}
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_ents_overhead_1000_day_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_fid_aves_overhead_1000_day_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_key_overhead_1000_day_1.png}}
    \caption{Optimal pump power results with 1000 km altitude—overhead mode: (a) the number of entanglement—nighttime, (b) the average fidelity—nighttime, (c) the number of keys—nighttime, (d) the number of entanglement—daytime, (e) the average fidelity—daytime, (f) the number of keys—daytime}
     \label{fig:op_pump_power_overhead_1000}
\end{figure}

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_ents_bisect_1000_night_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_fid_aves_bisect_1000_night_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_key_bisect_1000_night_1.png}}
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_ents_bisect_1000_day_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_fid_aves_bisect_1000_day_1.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/sampling_num_key_bisect_1000_day_1.png}}
    \caption{Optimal pump power results with 1000 km altitude—bisect mode: (a) the number of entanglement—nighttime, (b) the average fidelity—nighttime, (c) the number of keys—nighttime, (d) the number of entanglement—daytime, (e) the average fidelity—daytime, (f) the number of keys—daytime}
     \label{fig:op_pump_power_bisect_1000}
\end{figure}

%%wb, 3/16/2023, comment out for now; have replotted earlier on using more consistent colors
%%\input{results-under-optimal-pump-power}

\subsection{Key Generation Results}
\bing{3/16/2023: only plot the key rate. Also use effective key rate: total number of secret key bits/ total number of signals.}

\subsubsection{Satellite Altitude 500 km}

Total number of keys and key rate. x: number of days. plot 3 figures for  each: for the 3 difference distances; in each figure, show the 4 different schemes (asymptotic and finite, block and non-block) 2 modes separately.\\

The high ratio of the blockwise number of keys versus the non-blockwise number of keys with an altitude of 500 km and a distance of 1922 km is about $0.022\%$ in the overhead mode and $0.027\%$ in the bisect mode.

% \begin{figure}[h!]
%     \centering  \includegraphics[width=0.5\textwidth]{images/ideal_num_key_rate_500.png}
%     \caption{The number of secret keys and the key rate—altitude 500km. \bing{Left-most column, 3rd row, for the two finite-key cases, for 40 days, the key rate of the blockwise scheme is 0.6\% higher than the non-blockwise case. What is the number of keys for these two cases, and the sum of $B_i$'s for these two cases?}}
%     \label{fig:num_keys_rate_500}
% \end{figure}

\begin{figure}[h!]
    \centering
    \subfigure[]
    % width=0.155\textwidth
    {\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_overhead_10_551_500_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_overhead_10_1200_500_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_overhead_10_1922_500_0.png}}
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_bisect_10_551_500_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_bisect_10_1200_500_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_bisect_10_1922_500_0.png}}
    \caption{The effective key rate—altitude 500km: \bing{Left-most column, 3rd row, for the two finite-key cases, for 40 days, the key rate of the blockwise scheme is 0.6\% higher than the non-blockwise case. What is the number of keys for these two cases, and the sum of $B_i$'s for these two cases?} (a) overhead—baseline 551km, (b)overhead—baseline 1200km, (c)overhead—baseline 1922km, (d)bisect—baseline 551km, (e)bisect—baseline 1200km, (f)bisect—baseline 1922km.}
    \label{fig:eff_keys_rate_500}
\end{figure}

% \newpage

% \begin{figure}[h!]
%     \centering
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_551_500_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_1200_500_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_1922_500_0.png}}
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_551_500_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_1200_500_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_1922_500_0.png}}
%     \caption{The ratio of the blockwise number of keys versus the non-blockwise number of keys—altitude 500km: (a) overhead—baseline 551km, (b)overhead—baseline 1200km, (c)overhead—baseline 1922km, (d)bisect—baseline 551km, (e)bisect—baseline 1200km, (f)bisect—baseline 1922km.}
%     \label{fig:bk_nbk_ratio_500}
% \end{figure}

\begin{figure}[h!]
    \centering
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_551_500_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_1200_500_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_1922_500_0.png}}
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_551_500_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_1200_500_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_1922_500_0.png}}
    \caption{The ratio of the blockwise number of keys versus the non-blockwise number of keys—altitude 500km: (a) overhead—baseline 551km, (b) overhead—baseline 1200km, (c) overhead—baseline 1922km, (d) bisect—baseline 551km, (e) bisect—baseline 1200km, (f) bisect—baseline 1922km.}
    \label{fig:bk_nbk_ratio_500}
\end{figure}

% \newpage

\subsubsection{Satellite Altitude 800 km}

The high ratio of the blockwise number of keys versus the non-blockwise number of keys with an altitude of 800 km and a distance of 1922 km is about $0.064$ in the overhead mode and $0.7$ in the bisect mode.

\begin{figure}[h!]
    \centering
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_overhead_10_551_800_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_overhead_10_1200_800_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_overhead_10_1922_800_0.png}}
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_bisect_10_551_800_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_bisect_10_1200_800_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_bisect_10_1922_800_0.png}}
    \caption{The effective key rate—altitude 800km: (a) overhead—baseline 551km, (b)overhead—baseline 1200km, (c)overhead—baseline 1922km, (d)bisect—baseline 551km, (e)bisect—baseline 1200km, (f)bisect—baseline 1922km.}
    \label{fig:eff_keys_rate_800}
\end{figure}

% \newpage

% \begin{figure}[h!]
%     \centering
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_551_800_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_1200_800_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_1922_800_0.png}}
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_551_800_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_1200_800_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_1922_800_0.png}}
%     \caption{The ratio of the blockwise number of keys versus the non-blockwise number of keys—altitude 800km: (a) overhead—baseline 551km, (b)overhead—baseline 1200km, (c)overhead—baseline 1922km, (d)bisect—baseline 551km, (e)bisect—baseline 1200km, (f)bisect—baseline 1922km.}
%     \label{fig:bk_nbk_ratio_800}
% \end{figure}

\begin{figure}[h!]
    \centering
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_551_800_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_1200_800_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_1922_800_0.png}}
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_551_800_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_1200_800_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_1922_800_0.png}}
   \caption{The ratio of the blockwise number of keys versus the non-blockwise number of keys—altitude 800km: (a) overhead—baseline 551km, (b) overhead—baseline 1200km, (c) overhead—baseline 1922km, (d) bisect—baseline 551km, (e) bisect—baseline 1200km, (f) bisect—baseline 1922km.}
    \label{fig:bk_nbk_ratio_800}
\end{figure}

% \newpage

\subsubsection{Satellite Altitude 1000 km}
The high ratio of the blockwise number of keys versus the non-blockwise number of keys with an altitude of 1000 km and a distance of 1922 km is about $0.5$ in the overhead mode and $2.3$ in the bisect mode.
\begin{figure}[h!]
    \centering
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_overhead_10_551_1000_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_overhead_10_1200_1000_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_overhead_10_1922_1000_0.png}}
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_bisect_10_551_1000_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_bisect_10_1200_1000_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_eff_key_rate_bisect_10_1922_1000_0.png}}
    \caption{The effective key rate—altitude 1000km: (a) overhead—baseline 551km, (b)overhead—baseline 1200km, (c)overhead—baseline 1922km, (d)bisect—baseline 551km, (e)bisect—baseline 1200km, (f)bisect—baseline 1922km.}
    \label{fig:eff_keys_rate_1000}
\end{figure}

% \newpage

% \begin{figure}[h!]
%     \centering
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_551_1000_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_1200_1000_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_1922_1000_0.png}}
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_551_1000_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_1200_1000_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_1922_1000_0.png}}
%     \caption{The ratio of the blockwise number of keys versus the non-blockwise number of keys—altitude 1000km: (a) overhead—baseline 551km, (b)overhead—baseline 1200km, (c)overhead—baseline 1922km, (d)bisect—baseline 551km, (e)bisect—baseline 1200km, (f)bisect—baseline 1922km.}
%     \label{fig:bk_nbk_ratio_1000}
% \end{figure}

\begin{figure}[h!]
    \centering
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_551_1000_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_1200_1000_0.png}}
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_overhead_10_1922_1000_0.png}}
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_551_1000_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_1200_1000_0.png}} 
    \subfigure[]{\includegraphics[width=0.155\textwidth]{images/bk_nbk_ratio_bisect_10_1922_1000_0.png}}
    \caption{The ratio of the blockwise number of keys versus the non-blockwise number of keys—altitude 1000km: (a) overhead—baseline 551km, (b) overhead—baseline 1200km, (c) overhead—baseline 1922km, (d) bisect—baseline 551km, (e) bisect—baseline 1200km, (f) bisect—baseline 1922km.}
    \label{fig:bk_nbk_ratio_1000}
\end{figure}


\newpage

\subsection{Optimal Sampling rate}
For each block, nighttime and daytime, we set up a sample size $m_{i}\in\{10^3,5\times 10^3,10^4,5\times10^4,10^5,5\times10^5,10^6,5\times10^6,10^7,5\times10^7\}$ to find an optimal sample rate for the finite key distillation. For all altitudes and distances, the optimal sample size $m_{i}=5\times 10^{6}$ is to produce the maximum number of secret keys in the nighttime and daytime.

\subsubsection{Satellite Altitude 500 km}
For each figure, x-axis: \# of days, y-axis: optimal sampling rate (from 1\% to 50\%). Three curves: blockwise daytime and nighttime and non-block finite key. For the cases where we do not have a positive key rate for daytime (distance of 1922km, altitude of 800 and 1000km), just set it to 0.5 or some constant for now.  

\subsubsection{Satellite Altitude 800 km}

\subsubsection{Satellite Altitude 1000 km}
% \begin{figure}
%     \centering
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_overhead_10_551_500_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_overhead_10_1200_500_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_overhead_10_1922_500_0.png}}
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_bisect_10_551_500_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_bisect_10_1200_500_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_bisect_10_1922_500_0.png}}
%     \caption{Optimal sampling rate—altitude 500km. \bing{3/20/2023: use log scale for y-axis. In addition, the choice of the sampling rate: it looks like that the minimum value you used is 0.01; I think we should also allow $10^{-3}$, $10^{-4}$, $10^{-5}$ and $10^{-6}$; Walter's journal paper says $1/\sqrt{N}$, right? Anyway, we should discuss the choice of the sampling rate in the text and decide it correspondingly in the evaluation.}(a) overhead—baseline 551km, (b)overhead—baseline 1200km, (c)overhead—baseline 1922km, (d)bisect—baseline 551km, (e)bisect—baseline 1200km, (f)bisect—baseline 1922km.}
%     \label{fig:op_sampling_rate_500}
% \end{figure}

% \subsubsection{Satellite Altitude 800 km}
% \begin{figure}
%     \centering
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_overhead_10_551_800_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_overhead_10_1200_800_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_overhead_10_1922_800_0.png}}
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_bisect_10_551_800_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_bisect_10_1200_800_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_bisect_10_1922_800_0.png}}
%     \caption{Optimal sampling rate—altitude 800km. (a) overhead—baseline 551km, (b)overhead—baseline 1200km, (c)overhead—baseline 1922km, (d)bisect—baseline 551km, (e)bisect—baseline 1200km, (f)bisect—baseline 1922km.}
%     \label{fig:op_sampling_rate_800}
% \end{figure}

% \subsubsection{Satellite Altitude 1000 km}
% \begin{figure}
%     \centering
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_overhead_10_551_1000_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_overhead_10_1200_1000_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_overhead_10_1922_1000_0.png}}
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_bisect_10_551_1000_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_bisect_10_1200_1000_0.png}} 
%     \subfigure[]{\includegraphics[width=0.155\textwidth]{images/ideal_sample_rates_bisect_10_1922_1000_0.png}}
%     \caption{Optimal sampling rate—altitude 1000km. (a) overhead—baseline 551km, (b)overhead—baseline 1200km, (c)overhead—baseline 1922km, (d)bisect—baseline 551km, (e)bisect—baseline 1200km, (f)bisect—baseline 1922km.}
%     \label{fig:op_sampling_rate_1000}
% \end{figure}

==> protocol.tex <==
\section{Our Protocol}
The block-wise and entanglement-based BB-84 (E91) protocol runs as follows:
\begin{enumerate}
    \item A satellite, $s$, prepares a quantum state $\ket{\phi_{0}}\in \mathcal{H}_{g_{1}}\otimes \mathcal{H}_{g_{2}}\otimes \mathcal{H}_{E}$, where $\mathcal{H}_{g_{1}}\cong\mathcal{H}_{g_{2}}\cong \mathcal{H}_{d}^{\otimes B}$. Note that $B$ is the entire number of quantum states generated from the satellite such that $B=\sum_{i=1}^{n}B_{i}$ and $B_{i} = m_{i}+n_{i}$. The $g_{1}$ portion is sent to a ground station $g_{1}$ and the $g_{2}$ portion is sent to another ground station $g_{2}$ via the free space and atmospheric layer. 
    \item For each block period $i$, the station $g_{1}$ chooses a random subset $t_{i}$ of size $m_{i}$ out of $B_{i}$ and sends it to another station $g_{2}$. Both ground stations measure their systems indexed by $t_{i}$ in the X-measurement, which produces outcomes $q_{1}^{(i)}, q_{2}^{(i)}\in \mathcal{A}_{2}^{m_{i}}$, respectively. These values are revealed to each other via the authenticated channel.
    \item After the sampling and for each block period $i$, a pair of grounds stations, $(g_{1},g_{2})$, measures the $n_{i}$-number of the remaining portion of their system in the Z-measurement, which outputs their raw-keys $r_{1}^{(i)}$ and $r_{2}^{(i)}$ of size at most $n_{i}$ bits each. If there are observations of vacuum states, $\ket{vac}$, those will not contribute to the raw key so their keys are possibly smaller than $n_{i}$ in a lossy channel. Then these stations move to the next block and repeat processes $2$ and $3$ until they exhaust all the $n$-number of blocks.
    \item After all recurrences, $g_{1}$ and $g_{2}$ run an error correction protocol that can correct their block-wise all raw keys up to $Q$ errors, which reveals $leak_{EC}$ bits to Eve.
    \item Finally, privacy amplification operates on the error-corrected raw key resulting in their secret key.
\end{enumerate}

==> results-under-optimal-pump-power.tex <==
\subsection{Results under Optimal Pump Power}
overhead: 3 plots. Plot the optimal pump power, $B_i$, and fidelity 
%noise rate 
under the optimal pump power. x-axis: distance between ground stations (551, 1200, and 1922km). Each plot has 6 curves: for altitude 500km, 800km and 1000km, night time and day time. 

bisect: also 3 plots. 

Try to make sense the total number of secret keys and key rate (total number of secret keys / $\sum_i B_i$).   

\subsubsection{Non-blockwise asymptotic data:}

\begin{figure}[H]
    \centering  \includegraphics[width=0.5\textwidth]{images/nbk_asymp_data.png}
    \caption{Non-blockwise asymptotic data.}
    % \label{fig:op_pump_power_1000}
\end{figure}

\subsubsection{Non-blockwise sampling data:}
\begin{figure}[H]
    \centering  \includegraphics[width=0.5\textwidth]{images/nbk_sampling_data.png}
    \caption{Non-blockwise sampling data.}
    % \label{fig:op_pump_power_1000}
\end{figure}

\subsubsection{Blockwise asymptotic data:}
\begin{figure}[H]
    \centering  \includegraphics[width=0.5\textwidth]{images/bk_asymp_data.png}
    \caption{Blockwise asymptotic data.}
    % \label{fig:op_pump_power_1000}
\end{figure}

\subsubsection{Blockwise sampling data:}
\begin{figure}[H]
    \centering  \includegraphics[width=0.5\textwidth]{images/bk_sampling_data.png}
    \caption{Blockwise samplign data.}
    % \label{fig:op_pump_power_1000}
\end{figure}


